Radiative corrections and threshold resummed predictions to pseudoscalar Higgs boson production in QCD

This thesis studies the pseudoscalar Higgs boson production via gluon fusion in the EFT framework in a CP-conserving model. First, it presents the di-pseudoscalar Higgs boson production cross-section via gluon fusion till NNLO with the results valid for the pseudoscalar Higgs boson of MSSM and 2HDM with small tan $\beta$ by adjusting the top Yukawa coupling. We have used dimensional regularization to regulate the UV and IR divergences while carefully treating the Levi-Civita tensor and $\gamma_5$. Unlike the amplitudes involving a pair of scalar Higgs bosons, we do not need UV contact counter terms. We used Catani's predictions to factorize the IR singularities, and our IR poles agreed with Catani's predictions. Our results are essential for studies on producing a pair of pseudoscalar Higgs bosons at the LHC up to NNLO accuracy. This thesis also includes the next-to-soft-virtual (NSV) resummed corrections to $\overline{\text{NNLL}}$ accuracy, which are also matched to the NNLO cross-sections for a pseudoscalar Higgs boson production via gluon fusion. These NSV corrections are potentially significant compared to the conventional soft-virtual (SV) logarithms. We have estimated the uncertainties due to the choice of various PDFs and those due to the renormalization and factorization scales. The scale uncertainties show improvement for renormalization scale variation only, which suggests that NSV contributions from other parton channels and beyond NSV contributions in the gluon fusion channel are necessary for improved stability. We also studied the production cross-sections for mixed scalar-pseudoscalar states and their impact on QCD cross-sections for different values of the mixing angle $\alpha$. The study indicates the necessity of improving the precision results for the pseudoscalar Higgs boson up to an order comparable to that of the scalar Higgs boson.

==> Synopsis.tex <==
\chapter*{Synopsis}
\addcontentsline{toc}{chapter}{Synopsis}

The discovery of the long-awaited ``Higgs boson'' in 2012 was a crowning moment for one of the most remarkably successful fundamental theories of all time - the Standard Model (SM) of particle physics.
This discovery has opened up many possibilities, and exploring them requires precise theoretical predictions within the SM and beyond (BSM) in conjunction with revolutionary experimental progress.
So, the high-energy physics community is expecting new physics to show up as tiny deviations from the SM predictions by improving on the existing precision studies, probing the top and Higgs sectors, and looking for exotic signatures or even a new Higgs boson!

Perturbation theory is one of the most successful and celebrated methodologies to perform these precision calculations within the framework of the SM and beyond.
This theory allows the observable under consideration to be expanded in powers of a coupling constant.
The result obtained from the first term of such a perturbative series is called the leading order (LO) contribution, the next one is called the next-to-leading order (NLO) and so on.
In most cases, the LO results only give an idea of the order of magnitude but fail miserably to deliver a reliable theoretical prediction of the concerned observable(s).
So, one must go beyond the wall of the LO results to achieve higher accuracy and stability.
%
%The SM incorporates three of the four fundamental forces - electromagnetic $(\alpha_{EM})$, weak $(\alpha_{EW})$, and strong $(\alpha_\text{s})$.
Particle physicists can expand an observable in this theory in powers of the appropriate coupling constant associated with one of the three fundamental forces that SM incorporates, and perform perturbative calculations for each of these constants.
However, at typical energy scales where the hadron colliders operate, the contributions arising from the expansion of the strong coupling constant, $\alpha_\text{s}$, dominate over the others as it becomes exceedingly small in this region.
This serves as a motivation to expand $\alpha_\text{s}$ and evaluate terms beyond the LO to catch dominant contributions.

Quantum Chromodynamics (QCD) radiative corrections or perturbative QCD (pQCD) describes the study of these contributions as a series of the strong coupling constant, $\alpha_\text{s}$.
In addition, pQCD predictions depend on two unphysical scales, the renormalisation $(\mu_R)$ and factorisation $(\mu_F)$ scales, which get introduced in the process of renormalising the theory.
The truncation of the perturbative series at a particular order makes the fixed-order (FO) computations dependent on these unphysical scales.
This dependency decreases gradually as we include the series' contributions from higher and higher orders.
Hence, to make reliable theoretical predictions, it is necessary to consider the contributions from higher-order QCD corrections to any observable at the hadron colliders.


Unfortunately, it is widely known that the SM fails to explain certain natural phenomena such as the baryon asymmetry in the universe, the existence of dark matter, CP violation and so on.
%Most of these problems can be attempted to be solved by introducing more complex models like those including more particles and even more Higgs fields.
Another relevant question following the discovery of the Higgs boson is whether this scalar is the only one of its type as predicted by the SM or the first to have been discovered in a family of more such species from an underlying extended scalar sector.
So, the extension of the SM scalar sector by introducing more complex models is a common practice in constructing BSM physics.
Attempts are being made to relate the available Higgs data with BSM Higgs physics by extending the SM and adding another singlet field or a Higgs doublet.
The Minimal Supersymmetric extension of the Standard Model (MSSM) results from one such attempt.
Current experimental uncertainties suggest that the discovered Higgs is compatible not only with the SM predictions but also with the Higgs sector in the MSSM.
However, venturing these areas require precise predictions of relevant observables for scalar and pseudoscalar Higgs bosons.
The SM Higgs boson production cross-section is known to have unprecedented accuracy in pQCD in the Effective Field Theory (EFT) framework.
However, predictions for the pseudoscalar Higgs boson production still need to catch up.


\textit{
This thesis addresses precisely this context.
The central part of this thesis aims to calculate perturbative corrections to the production cross-section of the pseudoscalar Higgs boson in the framework of EFT.
This requires resumming the whole perturbative series for large logarithmic contributions near the threshold, in addition to computing the FO corrections.
The works included in the thesis are also expected to shed light on the aspect that resummation is as indispensable as FO corrections for accurate phenomenological predictions.
%In the subsequent discussions, we will concentrate on these two types of computations.
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Two loop QCD amplitudes for di-pseudo scalar production in gluon fusion}

%The inclusive cross-section for producing a pseudoscalar Higgs boson is known only up to NNLO order in pQCD, unlike that of a scalar Higgs boson production which is known up to N$^3$LO.
%Additionally,
Pair production of the pseudoscalar Higgs boson is essential to understand the nature of the extended Higgs sector along with that of a single pseudoscalar.
So, the first work I did involve computing the radiative corrections to the four-point amplitude,  $g+g \rightarrow A+A$, in massless QCD up to order $a_s^4$ in pQCD \cite{Bhattacharya_2020}.
We used EFT, which describes the coupling of pseudoscalar Higgs bosons to gluons and quarks directly in the large top quark mass limit.
We computed this for the gluon channel as a first step because of it being the dominant contribution.
And we chose the EFT framework because the number of loops increases computational complexities and so, such a choice enables physicists to go beyond NLO accuracy with the available tools and make precise and stable predictions with respect to the unphysical scales.
At the NNLO, two-loop virtual, one-loop single-real emission and double-real emission amplitudes are required.
In this article, as a first step towards going beyond NLO QCD corrections, we compute all the one- and two-loop amplitudes contributing to the pure virtual part of the cross-section for di-pseudoscalar production through gluon fusion.
The first step involved splitting the amplitude into two Lorentz- and gauge-invariant parts using the standard approach of the Projector method \cite{Banerjee2018}.
Consequently, the NNLO computations became doable as they are usually pretty cumbersome.
We have used dimensional regularisation and performed ultraviolet (UV) renormalisation to obtain the UV finite results.
Even then, the computation proved challenging as pseudoscalar Higgs boson couples to SM fields through two composite operators, which mix under renormalisation.
They also involve Levi-Civita tensor and $\gamma_5$, which are hard to define in dimensional regularisation.
So, the computation involves a careful treatment of the chiral quantities in dimensional regularisation.
Finally, the UV finite results were consistent with the universal infrared (IR) structure of QCD amplitudes \cite{Catani:1998bh}.
We obtained the finite amplitude by performing loop integrals and simplifications using packages like QGRAF, FORM, LiteRed, Reduze and Mathematica \cite{Nogueira:1991ex,Vermaseren:2000nd,vonManteuffel:2012np}.
%
Since we could compute only the amplitude in terms of two separate scalar coefficients because of the large data sizes being generated, we could not make further numerical analysis here.
However, the IR finite part of these amplitudes constitutes a vital component of any NNLO corrections to observables involving a pair of pseudoscalars at the Large Hadron Collider (LHC).
These results can be used in future for further phenomenological studies related to this process.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{NSV resummation for pseudoscalar higgs boson production at NNLO$+\overline{\text{NNLL}}$}

However, these FO QCD predictions have limited applicability because of certain large logarithmic contributions that arise in the threshold region of the kinematic phase space.
This region witnesses the emission of soft gluons giving rise to large logarithmic contributions to the cross-section when the partonic centre-of-mass energy approaches the pseudoscalar mass $(m_A)$.
Resumming these large logarithms to all orders in perturbation theory can solve the problem of unreliable FO predictions.
Additionally, the precise contribution of these parton-level logarithms to the hadron-level cross-section depends on the corresponding parton fluxes in that region.
For example, the associated gluon flux is large in the case of the discovered Higgs mass region of 125 GeV.
Hence, the threshold logarithms become significant due to the soft and collinear gluons.
The first soft-virtual term in a resummed expansion is known as the leading logarithm (LL), the next as the next-to-leading logarithm (NLL) and so on.
Unfortunately, at higher orders in QCD, these threshold corrections fail to complement the full FO results alone, and the role of the next-to-soft-plus-virtual (NSV) terms becomes significant.
These NSV contributions can, in principle, originate from parton channels other than the one corresponding to the Born contribution.
The nomenclature for these NSV terms is $\overline{\text{LL}}$, $\overline{\text{NLL}}$ and so on.
%
The scalar Higgs boson production computations have reached an accuracy of N$^3$LO level in the FO results and ${\text{N}^3\text{LL}}$ in the corresponding threshold resummed results.
The pseudoscalar production cross-sections are available to NNLO accuracy in QCD along with an approximate computation of three-loop threshold corrections \cite{Ravindran_2003,2016,Ahmed_2015}.


So, my subsequent work focussed on the resummation of Next-to-Soft Virtual (NSV) logarithmic terms for the threshold production of the pseudoscalar Higgs boson through gluon fusion at the LHC to $\overline{\text{NNLL}}$ accuracy \cite{Bhattacharya:2021hae}.
We resummed the SV and NSV logarithms to the desired order and matched them to the FO NNLO cross-sections.
The formalism we employed for this purpose used several contemporary designs to incorporate contributions from diagonal partonic channels and performed the resummation of the large logarithms to all orders \cite{ajjath2020soft}.
Using this framework, we obtained the resummed analytical results till $\mathcal{O}(a_s^2)$ and further studied their phenomenological implications.
We observed that these NSV logarithms are significant compared to the conventional SV logs.
We could study this from the K-factor values of the order-by-order results for the process under study.
For a clearer picture, we studied theory uncertainties and the impact of QCD corrections on mixed scalar-pseudoscalar states.
We observed that the renormalisation scale uncertainties decrease with the inclusion of NSV corrections.
This observation was in contrast with those from the seven-point scale uncertainties and the factorisation scale uncertainties where the uncertainties increased on including the NSV corrections.
These hinted at the significance of including other partonic channels for the NSV resummation and even beyond next-to soft-plus-virtual (NSV) corrections for the $gg$ channel being studied.
We also studied the effects of the other partonic channels on the resummed corrections till NNLO+$\overline{\text{NNLL}}$, compared to the $gg$ channel that we focus on in our work.
This also helped us to predict a source for the increase in uncertainties in the seven-point scale variation and factorisation scale variation results.
Additionally, we observed that precise theoretical estimates are needed to predict the mixing between scalar and pseudoscalar Higgs bosons, as the corrections only affected the mixing parameter by a few per cent.
However, this mixing was studied only for the $2\rightarrow1$ subprocess of pseudoscalar production \textit{via} gluon fusion and as per studies, the simple rescaling we have assumed in our studies will be modified if decay channels of the scalar/pseudoscalar Higgs is considered.
We have also studied the PDF uncertainties for the following choices of PDFs: NNPDF30, PDF4LHC15, HERAPDF20, CT14 and ABMP16 normalized with the corresponding results obtained from our default choice of MMHT 2014 PDF set, and presented the results for the production cross-section at NNLO+$\overline{\text{NNLL}}$.
We observed that w.r.t. to MMHT 2014 PDF set, the CT14 PDF set shows the least uncertainty.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this concluding paragraph, I would state that this thesis deals with higher-order QCD corrections to the observables associated with the pseudoscalar Higgs boson production.
I have performed the computations using our in-house codes and state-of-the-art techniques.
Although this thesis includes only the contribution of the gluon channel, we plan to consider contributions from the other parton channels in future works.
This is important because no matter how small, contributions from sub-dominant channels are also necessary along with the dominant ones to reduce dependency on the unphysical scales and make reliable predictions.
This is also observed in our uncertainty plots in the second project.
This thesis attempts to contribute to the computation of multi-loops and multi-legs, which play a central role in making precise theoretical predictions.
Notable developments in the techniques and methodologies to handle the complexities that arise with the increase in the number of loops and/or external particles have made these computations a reality.
The main tasks of the particle physics community can be primarily categorised into two parts now: testing the SM with unprecedented accuracy and searching for BSM physics.
We contribute to this task by means of a simple model in the effective field theory framework where the CP-odd Higgs boson is considered to be just another particle in addition to the CP-even Higgs boson in a CP-conserving model.
Herein lies the significance of this thesis.


==> frontpage_Original.tex <==
%\scalefont{1.1}
%\hspace{0pt}
%\vfill
\begin{center}
%
%{\Huge {\bf Precision QCD at the LHC}}
{\Large {\bf Radiative corrections and threshold resummed predictions to pseudoscalar Higgs boson production in QCD}}
%via gluon fusion
%
%\vskip 0.50cm
%
\\{\bf {\em By}}
%
\vskip 0.0cm
%
{\bf {\normalsize ARUNIMA BHATTACHARYA}}
%
\vskip 0.0cm
%
{\bf {\normalsize PHYS05201704009}}
%
\vskip 0.3cm
%
{\bf {\normalsize Saha Institute of Nuclear Physics, Kolkata}}
%
\vskip 0.5cm
%
{\textit{\normalsize A thesis submitted to the
%
\vskip 0.05cm
%
Board of Studies in Physical Sciences
%
\vskip 0.05cm
%
In partial fulfillment of requirements
%
\vskip 0.05cm
%
for the Degree of 
}}
%
\vskip 0.05cm
%
{\bf {\normalsize DOCTOR OF PHILOSOPHY}}
%
\vskip 0.1cm
%
{\textit{of}}
%
\vskip 0.1cm
%
{\bf {\normalsize HOMI BHABHA NATIONAL INSTITUTE}}
%
\vskip 0.7cm
%
\includegraphics[scale=0.56,keepaspectratio=true]{university.png}
% university.png: 234x215 px, 72dpi, 8.26x7.58 cm, bb=0 0 234 215
%
\vskip 0.5cm
%
{\bf {\normalsize February 2023}}
%
\vfill
\end{center}
\hspace{0pt}
%\footnotetext{Version 4}
%
\vfill
%
\clearpage
\newpage
%
\
%
\newpage
%
%~ \vskip 0.7cm
%
\centerline{{\bf{\LARGE Homi Bhabha National Institute}}}
%
\vskip 0.3cm
%
\centerline{{\bf {\large Recommendations of the Viva Voce Board}}}
%
\vskip 0.05cm
%
As members of the Viva Voce Board, we certify that we have read the dissertation prepared by Ms. Arunima Bhattacharya entitled "Radiative corrections and threshold resummed predictions to pseudoscalar Higgs boson production in
QCD" and recommend that it maybe accepted as fulfilling the dissertation requirement for the Degree of Doctor of Philosophy.
%
\vskip 0.06cm
%
\underline{\hspace{12.0cm}} Date: $6^{\text{th}}$ June $2023$
%
\vskip -0.5cm
%
Chairman: Prof. Munshi Golam Mustafa

%
\vskip 0.06cm
%
\underline{\hspace{12.0cm}} Date: $6^{\text{th}}$ June $2023$
%
\vskip -0.5cm
%
Guide/Convener: Prof. Prakash Mathews
%
\vskip 0.06cm
%
\underline{\hspace{12.0cm}} Date: $6^{\text{th}}$ June $2023$
%
\vskip -0.5cm
%
Examiner: Prof. Ambresh Shivaji
%
\vskip 0.06cm
%
\underline{\hspace{12.0cm}} Date: $6^{\text{th}}$ June $2023$
%
\vskip -0.5cm
%
Member 1: Prof. Gautam Bhattacharyya
%
\vskip 0.06cm
%
\underline{\hspace{12.0cm}} Date: $6^{\text{th}}$ June $2023$
%
\vskip -0.5cm
%
Member 2: Prof. Debasish Banerjee
%
\vskip 0.06cm
%
\underline{\hspace{12.0cm}} Date: $6^{\text{th}}$ June $2023$
%
\vskip -0.5cm
%
Member 3: Prof. Dilip Kumar Ghosh
%
\vskip 0.05cm
%
\hspace{0.7cm} Final approval and acceptance of this dissertation is contingent upon the candidate's submission of the final copies of the
dissertation to HBNI.
%
\vskip -0.4cm
%
\hspace{0.7cm} I hereby certify that I have read this dissertation prepared under my direction and recommend that it may be accepted as fulfilling the dissertation requirement.
%
\vskip 0.1cm
%
{\bf Date:} $6^{\text{th}}$ June $2023$
%
%\vskip 0.05cm
%
\\{\bf Place:} SINP, Kolkata \hfill
%
Guide : Prof. Prakash Mathews\hspace{1.0cm}
%
\newpage
%
\
%
\newpage
%
\centerline{{\bf {\large STATEMENT BY AUTHOR}}}
%
\vskip 1.00cm
%
\doublespacing
%
This dissertation has been submitted in partial fulfillment of requirements for an advanced degree at Homi Bhabha National Institute (HBNI) and is deposited in the Library to be made available to borrowers under rules of the HBNI.
%
\vskip 0.6cm
%
Brief quotations from this dissertation are allowable without special
permission, provided that accurate acknowledgement of source is made.
Requests for permission for extended quotation from or reproduction of
this manuscript in whole or in part may be granted by the Competent
Authority of HBNI when in his or her judgement the proposed use of the
material is in the interests of scholarship. In all other instances,
however, permission must be obtained from the author.

\vskip 1.5cm

$~$\hspace{11.0cm}Signature

\vspace{5 mm}

$~$\hspace{10.2cm}Arunima Bhattacharya
%
\newpage
%
\
%
\newpage
%
~
\vskip 1.2cm
%
\centerline{{\bf{\large{DECLARATION}}}}
%
\vskip 1.2cm
%
I, hereby declare that the investigation presented in the thesis has been
carried out by me. The work is original and has not been submitted
earlier as a whole or in part for a degree / diploma at this or any
other Institution / University.
%
\vskip 2.0cm
%
\rightline{Signature \hspace{1.5cm}}

\vspace{5 mm}

\rightline{Arunima Bhattacharya \hspace{0.9cm}}
%
\newpage
%
\
%
\newpage
%
\centerline{{\bf {\large List of Publications arising from the thesis \footnote{As it is standard in the High Energy Physics Phenomenology (hep-ph) community the names of the authors on any paper appear in their alphabetical order.}}}}
{\bf {\large Journals}}
\begin{enumerate}
  \item Two loop QCD amplitudes for di-pseudo scalar production in gluon fusion.
  
  \textbf{Arunima Bhattacharya}, Maguni Mahakhud, Prakash Mathews and V. Ravindran.
  
  In: JHEP 02 (2020) 121. arXiv: 1909.08993 [hep-ph].

 \item Next to SV resummed prediction for pseudoscalar Higgs boson production at NNLO$+\overline{\text{NNLL}}$.
 
 \textbf{Arunima Bhattacharya}, M. C. Kumar, Prakash Mathews and V. Ravindran.

 In: Phys.Rev.D 105 (2022) 11, 116015. arXiv: 2112.02341 [hep-ph].
\end{enumerate}
%
\vskip 1.2cm
%
\centerline{{\bf {\large List of other publications (not included in the thesis).}}} 
%
\begin{enumerate}
  \item Two-Loop QCD Amplitudes for Di-pseudo Scalar Production in Gluon Fusion.

  \textbf{Arunima Bhattacharya}, Maguni Mahakhud, Prakash Mathews and V. Ravindran.

  In: Springer Proc.Phys. 277 (2022) 49-53, 24th DAE-BRNS High Energy Physics Symposium.
\end{enumerate}

%\newpage
%
\centerline{\bf {\large Conferences/Workshops attended}}
\begin{enumerate}
 \item{\textbf{The Myriad Colourful ways of understanding extreme QCD Matter}} -
 {Workshop at ICTS-TIFR, Bangalore, India,
 $1^\text{st} - 7^\text{th}$ April 2019.}
 %
 \item{\textbf{Madgraph School 2019}} -
 {School at The Institute of Mathematical Sciences (IMSc), Chennai, India, $18^\text{th} - 22^\text{th}$ November 2019.}
 %
 \item{\textbf{XXXIII SERB Main School}} -
 {School on Theoretical High Energy Physics at SGTB Khalsa College, New Delhi, India,
 $7^\text{th} - 26^\text{th}$ December 2019.}
 %
 \item{\textbf{XXIV DAE-BRNS Symposium on High Energy Physics}} -
  {Virtual symposium organized by the National Institute of Science Education and Research, Jatni, Odisha,
  $14^\text{th}$ - $18^\text{th}$ December 2020.}
  %
  \item{\textbf{$8^\text{th}$ International Workshop on High Precision for Hard Processes (HP2 2022)}} -
  {Conference at the Discovery Museum in Newcastle, UK, organized by IPPP, University of Durham,
  $20^\text{th} - 22^\text{nd}$ September 2022.}
  %
  \item{\textbf{Baryons 2022 - International Conference on the Structure of Baryons}} -
  {Virtual conference at Seville, Spain,
  $7^\text{th} - 11^\text{th}$ November 2022.}
  %
  \item {\textbf{Computer Algebra with FORM for Developers 2023}} -
  {Workshop at IFT - UAM, Madrid, Spain, $12^{\text{th}} - 14^{\text{th}}$ April 2023.}
  %
  \item {\textbf{7th RED LHC workshop 2023}} -
  {Workshop at IFT - UAM, Madrid, Spain, $10^{\text{th}} - 12^{\text{th}}$ May 2023.}
\end{enumerate}
%
%\newpage
%
\centerline{\bf {\large Presentation/Poster}}
\begin{enumerate}
 \item{\textbf{XXIV DAE-BRNS Symposium on High Energy Physics} - }
  {"Two-loop QCD amplitudes for di-pseudo scalar production in gluon fusion",
  virtual symposium organized by the National Institute of Science Education and Research, Jatni, Odisha,
  $14^\text{th} - 18^\text{th}$ December 2020.}

  \item{\textbf{$8^\text{th}$ International Workshop on High Precision for Hard Processes (HP2 2022)}} -
  {"Next-to-soft-virtual resummed prediction for pseudoscalar Higgs boson production at NNLO$+\overline{\text{NNLL}}$",
  Discovery Museum in Newcastle, UK, organized by IPPP, University of Durham,
  $20^\text{th} - 22^\text{nd}$ September 2022.}

  \item{\textbf{Baryons 2022 - International Conference on the Structure of Baryons}} -
  {"Next to SV resummed prediction for pseudoscalar Higgs boson production at NNLO$+\overline{\text{NNLL}}$",
  virtually conference at Seville, Spain, $7^\text{th} - 11^\text{th}$ November  2022.}
\end{enumerate}
%
\vfill
%
%\rightline{Signature}

\rightline{Arunima Bhattacharya}
%
%
\newpage
%
\
%
\newpage
%
\hspace{0pt}
\vfill
{\Fontskrivan\bfseries {\large {Dedicated to my beloved Ma \& Baba, and my husband,}}}
%
\vskip 3.0cm
\begin{flushright}
{\Fontskrivan\bfseries {\large {For their endless love, support and encouragement.}}}
%
\end{flushright}
%
\hspace{0pt}
\vfill
%
\newpage
%
\
%
\newpage
%
\vskip 1.0cm
%
\centerline{{\bf{\large ACKNOWLEDGEMENTS}}}
%
\vskip 0.5cm
%
\centerline{}
\input{Acknowledgements}
%
%\newpage
%

